Ultra-Low-Complexity, Non-Linear Processing for MU-MIMO Systems

Non-linear detection schemes can substantially improve the achievable throughput and connectivity capabilities of uplink MU-MIMO systems that employ linear detection. However, the complexity requirements of existing non-linear soft detectors that provide substantial gains compared to linear ones are at least an order of magnitude more complex, making their adoption challenging. In particular, joint soft information computation involves solving multiple vector minimization problems, each with a complexity that scales exponentially with the number of users. This work introduces a novel ultra-low-complexity, non-linear detection scheme that performs joint Detection and Approximate Reliability Estimation (DARE). For the first time, DARE can substantially improve the achievable throughput (e.g., 40%) with less than 2x the complexity of linear MMSE, making non-linear processing extremely practical. To enable this, DARE includes a novel procedure to approximate the reliability of the received bits based on the region of the received observable that can efficiently approach the accurately calculated soft detection performance. In addition, we show that DARE can achieve a better throughput than linear detection when using just half the base station antennas, resulting in substantial power savings (e.g., 500 W). Consequently, DARE is a very strong candidate for future power-efficient MU-MIMO developments, even in the case of software-based implementations, as in the case of emerging Open-RAN systems. Furthermore, DARE can achieve the throughput of the state-of-the-art non-linear detectors with complexity requirements that are orders of magnitude lower.

==> Introduction.tex <==
\section{Introduction}
 % 1. What is the problem?
    % 2. Why is it interesting and important?
    % 3. Why is it hard? (E.g., why do naive approaches fail?)
    % 4. Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)
    % 5. What are the key components of my approach and results? Also include any specific limitations. 


   % \textcolor{azure}{ 1. What is the problem?}
    
Due to their favorable complexity requirements, existing MIMO developments employ linear (e.g., MMSE) based detectors. Still, such detectors leave unexploited throughput and connectivity benefits, making them inefficient in current and next-generation communication systems. %In particular, linear detectors can deliver acceptable throughput performance only when the MIMO channel matrix is well-conditioned \cite{nikitopoulos2014geosphere}. 
In particular, the achievable throughput by linear detection is severely degraded when the MIMO channel matrix is poorly conditioned \cite{nikitopoulos2014geosphere,Antipodal}. For example, such channels occur when the number of transmitted streams is close to the number of receiver antennas.  
This limitation has led to massive MIMO systems where the base station antennas are much larger than the supported number of streams. However, a massive number of base station antennas (e.g., 128) requires a massive number of RF chains that consume excessive power to support a relatively small number of streams (e.g., 12). %\textcolor{red}{Give an example of the power consumed only from }  %Linear detection involves a linear transformation, transforming the MIMO interfering channel into several non-interfering ones. However, this linear transformation severely degrades the capabilities of the MIMO channel. Such limitations of linear processing have resulted in massive MIMO systems with high power consumption where a massive number of base station antennas (e.g., 64) and RF chains are required to support a smaller number of streams (e.g., 8).
%For example, an RF chain can typically consume $15.6$ W, resulting in an increase in power consumption of $500$W from a $32-$antenna to a $64-$antenna base station.

% 2. Why is it interesting and important?
% 3. Why is it hard? (E.g., why do naive approaches fail?)




%\textcolor{azure}{3. Why is it hard? (E.g., why do naive approaches fail?)}

 In contrast, non-linear detection can overcome the limitations imposed by linear detection and provide substantial throughput and connectivity gains compared to linear detection. \textcolor{red}{Cite our corresponding work}. In Section \ref{s:Eval}, we elaborate that non-linear detection can deliver better throughput than linear detection while significantly reducing the number of base station antennas and, therefore, RF chains. As a result, the power consumption of a base station can be reduced substantially by employing non-linear processing.   However, the complexity requirements of the joint soft information computation (e.g., in the form of Log-Likelihood Ratios) are still substantially higher than linear processing for a large number of concurrently transmitted streams. 
 This is because joint soft information computation typically involves solving multiple minimization problems, each with a worst-case complexity that scales exponentially with the number of users. %For example, the approach of \cite{softAPPmimo} requires multiplications of the order of $10^{14}$ for a $16\times12$ MIMO system per channel use \textcolor{black}{(e.g., per resource element and time-domain symbol)}. 
 Many approximate non-linear detection schemes exist. However, schemes that are based on message passing algorithm \cite{CHEST}, local neighborhood search \cite{LAS,ULAS}, and convex optimization \cite{lowdet} are too complex since the processing complexity requirements per received vector samples when accumulated are substantially higher than of per channel update processing (e.g., inversion) for MMSE. 
 %However, schemes that are based on message passing algorithm \cite{CHEST}, local neighborhood search \cite{LAS,ULAS}, and convex optimization
 Furthermore, the achievable performance of schemes such as \cite{LAS,ULAS} significantly degrade when transmitting dense symbol constellations (e.g., 64 QAM). In addition, the performance of message passing \cite{CHEST} is highly dependent on the statistics of large systems.

% 4. Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?)
%Antipodal detection and decoding principle introduced in \cite{Antipodal} can outperform existing non-linear detection schemes with a better performance complexity tradeoff. However, current Antipodal approaches rely on statistics of large systems and become approximate for a smaller number of streams. Furthermore, the current Antipodal approach accepts or discards the whole vector. Therefore, it may discard symbol (and therefore bit) estimates of all users as unreliable for a particular realization, while some symbols (and therefore bits) (e.g., of strong users) could still be reliable. In addition, current Antipodal approaches are strictly based on sequential hard sphere decoders (SD). 

%On the other hand, parallelizable SD schemes with a fixed complexity and latency, such as k-best SDs and fixed-complexity SDs, target the worst-case transmission condition resulting in high computational complexity requirements. In addition, k-best SDs require large k values and extensive long sorting operations that compromise their implementation efficiency. In this direction, the massively parallelizable tree search-based detection scheme can focus the available processing power on the most promising solutions to the non-linear detection problem based on the transmission channel. Although this scheme has shown a complexity performance tradeoff better than other non-linear detection schemes, its complexity requirements are still significantly higher than linear detection.

 %A well-designed tradeoff between sequential and parallelizable schemes needs to be exploited to realize the gains of non-linear detection with comparable complexity and latency requirements to linear detection. In this work, we exploit a tradeoff between sequential and parallel tree search to introduce a novel tree search-based algorithm which can provide substantial throughput (e.g., $40\%$) and connectivity benefits with comparable complexity (e.g., $2\times$) and latency requirements to that of linear detection.
 %In particular, this paper introduces a simple detection scheme that performs Approximate Reliability Estimation  (\systemname).\systemname is a novel detector structure that provides bit reliability information based on the region of the received observable while exploiting a fine tradeoff between sequential and parallel tree search. Consequently, \systemname can compute reliability information in a hardware-friendly manner while avoiding any sorting operations, which is a bottleneck for existing non-linear detectors \cite{Shabany08,KbestGuo}. In contrast to the Antipodal approach, \systemnameapplies to a smaller number of streams, determines the reliability of bits per user basis (and does not characterize the whole vector), and has a fixed maximum processing latency.In particular, Section  provides the details of \systemname. \systemname can efficiently quantize the reliability information as a function of complexity, providing a flexible performance/complexity tradeoff. Due to this, \systemname can approximate the optimal soft information computation with lower complexity than exiting non-linear detectors that provide hard estimates. As validated by simulation evaluations in Section , \systemname is the first scheme that can significantly outperform the MMSE detector (e.g., throughput gains of 50\% even in massive MIMO scenarios) with comparable complexity.

%\textcolor{azure}{2. Why is it interesting and important?}

   With the popularity of the open-RAN paradigm,  power-efficient physical layer solutions that can enhance network performance are timely and necessary. Such solutions are required to meet the stringent latency requirements of the 3GPP physical layer, even in a softwarerized implementation. Therefore, a non-linear detection scheme that can substantially reduce the power consumption of a base station with ultra-low complexity requirements becomes an ideal candidate for modern physical layer developments. A practical non-linear detection scheme must ideally have a fixed latency and complexity and be capable of delivering substantial gains compared to linear detection, with a very small complexity increase. A comparable small complexity increase (e.g., $< 2\times$) can enable the exchange of linear detection with non-linear detection in exiting deployments without significant modifications to the architecture and without compromising the supported bandwidths and the number of user streams.


 %\textcolor{azure}{4. Why hasn't it been solved before? (Or, what's wrong with previous proposed solutions? How does mine differ?}
 
 Tree search-based sphere decoders (SD) are promising to achieve the optimal hard Maximum-Likelihood (ML) \cite{nikitopoulos2014geosphere} performance and soft detection performance in the MIMO uplink. All SD schemes consist of a channel matrix-dependent preprocessing stage and a per-received vector post-processing stage. The channel matrix-dependent preprocessing stage involves a triangular (e.g., QR) decomposition and is only required to be performed once the channel changes significantly, similar to the inversion of linear detection, and with similar complexity requirements. However,  the complexity requirements of the per-received vector post-processing stage in SD schemes are many orders of magnitude higher than that of linear processing \cite{FCSD,SFSD}. %Furthermore,  depth-first SDs are strictly sequential, and their latency and complexity requirements are random and become impractical for high-dimensional systems.   
 In this work,  we introduce Detection and Approximate Reliability Estimation  (\systemname):, a highly-efficient ultra-low-complexity non-linear detection scheme that, for the first time, can significantly outperform linear detection (e.g., throughput gains of 40\% even in massive MIMO scenarios) with a maximum complexity that is only $2 \times$ than linear detection. 
 %In this work, we focus on such non-linear detection schemes which can provide substantial gains in comparison to linear processing with comparable processing complexity and latency requirements. In particular, we focus on the complexity requirements per received vector sample, since the complexity of processing per channel update, such as the triangular decompositions necessary for non-linear processing and inversions for linear processing, are similar and can employ the same interpolation methods in time and frequency to reduce the complexity. In contrast, since linear detection involves transforming the MIMO channel into independent SISO channels, traditional methods employed to compute soft information in SISO channels can be applied directly. Therefore, reducing the computational complexity and the processing latency of the joint soft information computation problem to be comparable to that of linear detection is extremely challenging, and the available processing power must be focused on the solutions that significantly affect the accuracy of soft information.
 In contrast, the aforementioned existing detection schemes are at least an order of magnitude more complex than linear detection.
 In this context of low-complexity non-linear detection, the antipodal detection and decoding principle introduced in \cite{Antipodal} can outperform existing non-linear detection schemes with a better tradeoff between performance and complexity. However, current Antipodal approaches rely on statistics of large systems and become approximate for a smaller number of streams. Furthermore, the current Antipodal approach accepts or discards the whole vector. Therefore, it may discard symbol (and therefore bit) estimates of all users as unreliable for a particular realization, while some symbols (and therefore bits) (e.g., of strong users) could still be reliable. %In addition, current Antipodal approaches are strictly based on sequential hard sphere decoders (SD) with a random processing latency. 
 In contrast to the Antipodal approach, \systemname applies to a smaller number of streams, determines the reliability of bits per user basis (and does not characterize the whole vector), and has a fixed processing latency.
 
%

 %In this direction, the massively parallelizable non-linear (MPNL) detection scheme offers a flexible performance/ complexity trade-off and can approach Maximum-Likelihood (ML) detection performance, but typically requires many parallel processing elements. Although MPNL can approach ML detection performance, it underperforms when the complexity is restricted to be comparable (e.g., $2\times$) to linear processing. This is because MPNL enables massively parallel processing that avoids any dependencies required to approximate soft information efficiently.
% In the same context, the massively parallelizable non-linear (MPNL) detection scheme can minimize processing latency while achieving ML performance by dividing the detection process into parallel processes that do not interact. In contrast, \systemname exploits dependencies to maximize performance gains specifically for a smaller complexity.
 
%\textcolor{azure}{5. What are the key components of my approach and results? }
Section \ref{s:method}  provides the details of \systemname. \systemname can efficiently quantize the reliability information as a function of complexity, providing a flexible performance/complexity tradeoff. Due to this, \systemname can approximate the optimal soft information computation with lower complexity than exiting non-linear detectors that provide hard estimates. \systemname exploits a novel detector structure to provide soft bit reliability information based on the region of the received observable. Consequently, \systemname can compute reliability information in a hardware-friendly manner while avoiding any sorting operations, which is a bottleneck for existing non-linear detectors \cite{Shabany08,KbestGuo}. As a result, as we show in Section \ref{s:Eval}, \systemname can achieve substantial throughput gains while its complexity is only $2\times$ compared to linear MMSE. 
 %This paper introduces a scheme that performs Detection and Approximate Reliability Estimation  (\systemname).  .  As validated by simulation evaluations in Section , \systemname is the first scheme that can significantly outperform the MMSE detector (e.g., throughput gains of 50\% even in massive MIMO scenarios) with comparable complexity.
